Neural Video Coding under Limited Delay: Theoretical Optimality and System Design

Traditional neural video compression (NVC) methods predominantly follow strictly causal predictive-coding paradigm, treating zero-frame delay as a fixed constraint rather than delay as an explicit design parameter. From an information-theoretic perspective, allowing limited frame delay enables a codec to exploit correlations with future frames within the delay window, thereby reducing uncertainty that is inaccessible to strictly causal prediction and potentially improving the rate-distortion tradeoff. In this work, we formalize this intuition through a rigorous rate-distortion analysis builds on the clique factorization of Markov networks, and propose Graph-Factored Sequential Coding (GFSC), a principled framework for sequential video coding under limited delay. To our knowledge, we provide the first theoretical result showing that, for general $K$-order Markov sources with positive distributions, a $K$-frame delay is sufficient to attain joint-coding rate-distortion optimality over a nontrivial distortion region, a guarantee unavailable to zero-delay causal coding in general. In practice, we instantiate GFSC through lightweight neural modules, allowing existing causal predictive codecs to be augmented without modifying their core architectures. Experiments across multiple NVC models and datasets show that GFSC consistently improves rate-distortion performance over the corresponding causal counterparts. Under matched delay budgets, GFSC also achieves competitive performance compared with representative bidirectional codecs.

==> figs/fig-gate_visualize.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-1em}
\centering
\begin{minipage}[t]{\linewidth}
\centering

\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_1$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_1$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_1$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/w_t_t+1.jpeg}\vspace{-7pt}
    \caption*{\tiny $\bar{\omega}_{1,2}$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/w_t_t+2.jpeg}\vspace{-7pt}
    \caption*{\tiny $\bar{\omega}_{1,3}$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/w_t_t+3.jpeg}\vspace{-7pt}
    \caption*{\tiny $\bar{\omega}_{1,4}$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t+1.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_2$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t+2.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_3$}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{imgs/mcl_jcv_sample_2/X_t+3.jpeg}\vspace{-7pt}
    \caption*{\tiny $X_4$}
\end{subfigure}
% \vspace{2pt}
\begin{subfigure}{\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Delay & $K=1$ & $K=2$ & $K=3$ \\
\hline
PSNR (dB) & 36.59 &  37.40 & 38.77 \\
\hline
\end{tabular}
}
\end{subfigure}
\end{minipage}
\caption{Qualitative and quantitative results under different delay settings.
}
\label{fig:interpolation_vis}
\vspace{-2em}
\end{wrapfigure}

==> files/app-joint_coding_gaussian.tex <==

\section{Joint coding for Gaussian source}\label{app-sec:jc_gauss}


==> files/app-proof.tex <==


% Next, we show this coding scheme can still be strictly constructed following the system model in Section~\ref{subsec:system_model}. 
% For each $(j,k)$ with $k = \min\{j+K, L\}$, we introduce augmented variables
% \begin{equation}
%     \tilde{Y}_{j,k} \triangleq (X_j, \tilde{X}_{j,k}), 
%     \qquad 
%     V_{j,k} \triangleq (U_j, U_{j,k}),
% \end{equation}
% and replace $(\tilde{X}_{j,k}, U_{j,k})$ by $(\tilde{Y}_{j,k}, V_{j,k})$ in the coding system of Definition~\ref{app-def:vf_k_ird}. 
% This transformation preserves the Markov structure and functional dependencies of the original construction.
% Under this augmentation, the corresponding rate term can be decomposed as
% \begin{align}
%     I(\tilde{Y}_{j,k}; V_{j,k} \mid U_{\mathcal{E}^{(K)}_{j,k}})
%     &= I(X_j, \tilde{X}_{j,k}; U_j, U_{j,k} \mid U_{\mathcal{E}^{(K)}_{j,k}}) \\
%     &= I(\tilde{X}_{j,k}; U_{j,k} \mid U_{\mathcal{E}^{(K)}_{j,k}})
%     + I(X_j; U_j \mid U_{j,k}, U_{\mathcal{E}^{(K)}_{j,k}}),
% \end{align}
% where the second equality follows from the chain rule and Markov chain constraints.
% Therefore, introducing the additional variables $\{U_j\}_{j=1}^L$ does not alter the achievable sum-rate, and the coding scheme in Definition~\ref{app-def:vf_k_ird} continues to achieve the joint-coding optimality in high resolution regime. 

% Note that this result is strictly achieved in the asymptotic setting, and it is approximately achieved in the one-shot setting according to Theorem~\ref{app-thm:ope_rd_region}.




==> files/default_notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file. Use of this style is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}





==> tabs/app-tab-network_arch.tex <==
% \begin{table}[!ht]
% \centering
% \caption{Encoder, decoder, interpolation and conditioning modules for VCT-ISC.}
% \label{app-tab:network_arch}
% \begin{minipage}{0.45\linewidth}
%     \centering
%     \begin{tabular}{|c|}
%     \hline
%     Input ($3\times 256 \times 256$) \\
%     \hline
%     conv($3, 128, 5, 2, 1$), GDN($128$) \\
%     \hline
%     conv($128, 128, 5, 2, 1$), GDN($128$) \\
%     \hline
%     conv($128, 128, 5, 2, 1$), GDN($128$) \\
%     \hline
%     conv($128, d_{C}, 5, 2, 1$) \\
%     \hline
%     \end{tabular}
%     \caption*{(a) Encoder}
% \end{minipage}
% \hfill
% \begin{minipage}{0.45\linewidth}
%     \centering
%     \begin{tabular}{|c|}
%     \hline
%     Input ($d_C$) \\
%     \hline
%     upconv($d_C, 128, 5, 2, 1$), GDN($128$) \\
%     \hline 
%     upconv($128, 128, 5, 2, 1$), GDN($128$) \\
%     \hline
%     upconv($128, 128, 5, 2, 1$), GDN($128$) \\
%     \hline
%     upconv($128, 3, 5, 2, 1$) \\
%     \hline
%     \end{tabular}
%     \caption*{(b) Decoder}
% \end{minipage}
% \begin{minipage}{0.45\linewidth}
%     \centering
%     \begin{tabular}{|c|}
%     \hline
%     Input ($2\times d_C$) \\
%     \hline
%     conv($2\times d_C, 0.5 \times d_C, 3, 1, 1$) \\
%     \hline
%     LeakyReLU($0.01$) \\
%     \hline
%     conv($0.5 \times d_C, 1, 1, 1, 0$) \\
%     \hline
%     \end{tabular}
%     \caption*{(c) Interpolation gating module}
% \end{minipage}
% \hfill
% \begin{minipage}{0.45\linewidth}
%     \centering
%     \begin{tabular}{|c|}
%     \hline
%     Input ($2\times d_C$) \\
%     \hline
%     conv($2\times d_C, d_C, 1, 1, 1$), GDN($d_C$) \\
%     \hline 
%     conv($d_C, d_C, 3, 1, 1$), GDN($d_C$) \\
%     \hline
%     conv($d_C, d_C, 1, 1, 1$) \\
%     \hline
%     \end{tabular}
%     \caption*{(d) Conditioning module}
% \end{minipage}
% \end{table}


\begin{table*}[!t]
\centering
\caption{Delay fusion modules in the main and motion branches of DCVC.}
\label{tab:dcvc_delay_fusion}
\small

\begin{minipage}{0.49\textwidth}
    \centering
    \begin{tabular}{|p{0.96\linewidth}|}
        \hline
        \shortstack[l]{Input: current and delayed main latents
        $\mathbf{y}_t,\mathbf{y}_{t+1}\in
        \mathbb{R}^{96\times H_y\times W_y}$} \\
        \hline
        Stack two frames and partition into non-overlapping
        $4\times4$ spatial windows \\
        \hline
        Joint spatiotemporal tokens:
        $[B n_w,\;2\cdot4^2,\;96]$ \\
        \hline
        Add temporal and spatial positional embeddings \\
        \hline
        LayerNorm($96$) \\
        \hline
        4-head self-attention($96$), residual connection \\
        \hline
        LayerNorm($96$) \\
        \hline
        MLP: Linear($96,192$), GELU, Linear($192,96$),
        residual connection \\
        \hline
        Depthwise conv($96,96,3,1,1$, groups$=96$), GELU,
        residual connection; applied per frame \\
        \hline
        Repeat the attention--MLP--spatial-mixing block $\times 2$ \\
        \hline
        Conv($96,96,3,1,1$) and residual addition to $\mathbf{y}_t$ \\
        \hline
    \end{tabular}
    \caption*{(a) Main-branch spatial-temporal attention fusion}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
    \centering
    \begin{tabular}{|p{0.96\linewidth}|}
        \hline
        \shortstack[l]{Input: current and delayed motion features
        $\mathbf{m}_t,\mathbf{m}_{t+1}\in
        \mathbb{R}^{128\times H_m\times W_m}$} \\
        \hline
        Concatenate $\mathbf{m}_t$, $\mathbf{m}_{t+1}$, and
        $|\mathbf{m}_{t+1}-\mathbf{m}_t|$
        ($384$ channels) \\
        \hline
        Conv($384,128,1,1,0$) \\
        \hline
        LeakyReLU($0.1$) \\
        \hline
        Residual block($128$), repeated $\times 2$:
        conv($128,128,3,1,1$), LeakyReLU($0.1$),
        conv($128,128,3,1,1$), LeakyReLU($0.1$),
        residual addition \\
        \hline
        Conv($128,128,3,1,1$) \\
        \hline
        Add the predicted residual to $\mathbf{m}_t$ \\
        \hline
        Output: fused motion feature
        $\mathbf{m}_{\mathrm{fused}}\in
        \mathbb{R}^{128\times H_m\times W_m}$ \\
        \hline
    \end{tabular}
    \caption*{(b) Motion-branch neural CNN fusion}
\end{minipage}

\vspace{2pt}
\parbox{0.96\textwidth}{\footnotesize
Conv notation: $\mathrm{conv}(C_{\mathrm{in}},C_{\mathrm{out}},k,s,p)$
denotes a 2D convolution with kernel size $k$, stride $s$, and padding $p$.
The attention defaults are depth $=2$, window size $=4$, number of heads $=4$,
and MLP ratio $=2$. The delay-fusion modules are bypassed when the delayed
frame is not provided.}
\end{table*}





==> tabs/app-tab-per_frame_bd_rate.tex <==
\begin{table}[t]
\centering

\begin{minipage}{0.48\linewidth}
\centering
\caption{BD-rate (\%) comparison on UVG across different frames.}
\label{app-tab:bd_rate_perframe_uvg}
\begin{tabular}{|c|c|c|c|}
\hline
& Avg & $j=1$ & $j=32$ \\
\hline
Causal & 0.0 & 0.0 & 0.0 \\
\hline
Delay1 & -22.04 & -6.29 & -23.06 \\
\hline
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\centering
\caption{BD-rate (\%) comparison on UVG with different GOP sizes.}
\label{app-tab:bd_rate_gop_uvg}
\begin{tabular}{|c|c|c|c|}
\hline
& $8$ & $16$ & $32$ \\
\hline
Causal & 0.0 & 0.0 & 0.0 \\
\hline
Delay1 & -18.63 & -20.84 & -22.04 \\
\hline
\end{tabular}
\end{minipage}

\end{table}

==> tabs/tab-delayed_bd_rate.tex <==

\begin{table}[t]
\centering
\caption{BD-rate (\%) comparison between VCT-ISC and delayed coding baselines. 
Quantitative results correspond to Figure~\ref{fig:delayed_rd_curves}.
% Each group reports results for VCT, DHVC, and SSF, respectively.
}
\label{tab:delayed_bd_rate}
\begin{tabular}{|l|cc|cc|ccc|}
\hline
~ & \multicolumn{2}{c|}{ DCVC-B } & \multicolumn{2}{c|}{ HM-RA } & \multicolumn{3}{c|}{ ISC } \\
\cline{2-8}
Data & $K=1$ & $K=2$ & $K=1$ & $K=3$ & $K=1$ & $K=2$ & $K=3$ \\
\hline
UVG & -4.05 & -18.93 & -1.49 & -34.00 & -23.36 & -31.59 & -38.00 \\
\hline
MCL-JCV & -21.31 & -29.33 & 41.14 & 20.96 & -17.31 & -25.97 & -27.98 \\
\hline
\end{tabular}
% \vspace{-1em}
\end{table}

